Towards Efficient Active Learning of PDFA

We propose a new active learning algorithm for PDFA based on three main aspects: a congruence over states which takes into account next-symbol probability distributions, a quantization that copes with differences in distributions, and an efficient tree-based data structure. Experiments showed significant performance gains with respect to reference implementations.

==> WLStar.tex <==
\subsection{\PLstar}

%&\PLstar\ is an iterative learning algorithm that constructs a PDFA by interacting with a MAT teacher, that is, the teacher exposes two oracles \MQ\ and \EQ. And using an 
Here we present \PLstar, a variant of \WLstar~\cite{weiss_WFA_learning}. Similarly, it uses an observation table $O_{\Pref,\Suff}$ for storing outcomes of $\MQ_{\PLstar}$, where $\Pref \subset \Symb^\ast$ is the set of \emph{prefixes} (stored in row indices) and $\Suff \subset \{\terminal\}\cup\Symb^{+}$ is the set of \emph{suffixes} (stored in column indices). 
%
For every 
$p\in\Pref$ and $s\in\Suff$, $O_{\Pref,\Suff}[p,s] = \MQ_{\PLstar}(p s) = \policyL_{\staI}(p s)$, where $\policyL$ is defined in (\ref{eq:policyL}).
%
Unlike \WLstar, \Pref\ is divided in two parts~\cite{De_la_higuera:2010}, namely \emph{RED} which are the rows used to construct \emph{states}, and \emph{BLUE} which are the rows representing continuations. The algorithm ensures that for every row in \emph{RED} all its continuations are in \Pref.
%
\PLstar\ consists of three main steps. The first one expands $O_{\Pref,\Suff}$ through the use of $\MQ_{\PLstar}$\ until it becomes \emph{closed} and \emph{consistent}. The second one constructs a hypothesis automaton. The third one calls $\EQ_{\PLstar}$\ with the proposed hypothesis. These steps are repeated as long as $\EQ_{\PLstar}$\ yields a counterexample, otherwise it stops and returns the last hypothesis.

\textbf{Step 1: Observation table expansion}
To expand $O_{\Pref,\Suff}$, \PLstar\ uses \tol-equality to compare rows. For this, we extend the notation $\tequal$ to strings as follows: $p \tequal_{\Suff,\tol} p'$ if $\traW(p) \tequal_{\tol} \traW(p')$ restricted to the set \Suff, that is, \tol-equality is evaluated on prefixes $p, p'\in \Pref$ for every suffix $s \in \Suff$ of the observation table.
These properties are stated as follows:
\begin{itemize}
    \item Closedness: $\forall p \in BLUE$, $\exists p' \in RED$ s.t. $p \approx_{\Suff,\tol} p'$.
    \item Consistency: $\forall p, p' \in RED$ if $p \approx_{\Suff,\tol} p'$ then $\forall \symb \in \Symb$, $ p \symb \approx_{\Suff,\tol} p' \symb$.
\end{itemize}

\textbf{Step 2: PDFA construction}
Unlike \Lstar\, where a unique row in \emph{RED} represents a state, in \PLstar\ a state is a \emph{group} of \tol-equal rows. Since \tol-equality is not an equivalence relation, there is no natural unique way of grouping. \PLstar\ builds a partition going through the following three main steps\footnote{The major differences with \WLstar\ are that it partitions \Pref, while we partition only \emph{RED}, and it uses a different clustering technique.}:
\begin{enumerate}
    \item An initial partition \Clu\ is constructed in a greedy manner. If there is a single cluster such that $p$ is \tol-equal to all prefixes already in that cluster, then add $p$ to it. If more than one cluster exist, then add it to the one for which its Euclidean distance to the cluster's centroid\footnote{The centroid is the multivariate equivalent of the mean.} is minimal. Otherwise, create a new cluster for $p$\footnote{Notice that this way of grouping does not rely on an external clustering library}. \Clu\ satisfies the following property:
    \begin{description}
    \item[\tol-equality] $\forall p, p' \in RED$, if $\Clu(p) = \Clu(p')$ then $p \approx_{\Suff,\tol} p'$.
    \end{description}
%    
    \item Transitions are added as follows. We denote $\Ctrans \in \Clu \times \Symb \times \Clu$ the transition relation. For each $p \in RED$, for each $\symb \in \Symb$, if $p\symb \in RED$ we add a transition by $\symb$ from $\Clu(p)$ to $\Clu(p\symb )$, that is $(\Clu(p), \symb, \Clu(p\symb)) \in \Ctrans$. Otherwise, we find all groups in \Clu\ containing rows that are \tol-equal to $p\symb$. Since the table is closed, there is at least one such group. Then, a transition is added to the group $c^\ast$ which centroid is closest to $p\symb$, that is: $(\Clu(p), \symb, c^\ast) \in \Ctrans$. After transitions are added, the following property is satisfied:
    \begin{description}
    \item[Coverage] $\forall p\in RED, \symb\in\Symb$, $|\Ctrans(\Clu(p), \symb, \_))| \geq 1$.
    \end{description}
%    
    \item The partition \Clu\ is refined until the transition relation \Ctrans\ is deterministic.
    \begin{description}    
    \item[Determinism] $\forall p\in RED, \symb\in\Symb$, $|\Ctrans(\Clu(p), \symb, \_))| = 1$. 
    \end{description}
\end{enumerate}
%This algorithm not only ensures \tol-equality and determinism in the grouping, it also defines a complete function over $\Symb$, thus constructing a PDFA.
Now it is possible to construct a PDFA where the set of states is \Clu, the transition function is \Ctrans, and the probability distribution over symbols for each state is the centroid of the cluster restricted to \SymbT.

\textbf{Step 3: Answering $\EQ_{\PLstar}$}
%When the target system is a black box, determining exactly if the hypothesis is equivalent to the target becomes intractable. This is solved for LM-RNNs by sampling the target LM-RNN and hypothesis PDFA
%$A$ an arbitrary finite number of times, testing every prefix of each sample to see if it is a counterexample.
%In order to implement $\EQ_{\PLstar}$ 
We adapted Hopcroft-Karp algorithm for testing equivalence of DFA~\cite{hopcroft_karp} to PDFA. Starting from initial states and continuing in a BFS manner, states are compared using $L_\infty(\policy(\sta), \policy(\widehat{\sta})) \leq t$, where \sta\ is a state of the target PDFA \Aut\ and $\widehat{\sta}$ is a state of the hypothesis PDFA $\widehat{\Aut}$. 
%
When \Aut\ and $\widehat{\Aut}$ are found to be not \tol-equal, $\EQ_{\PLstar}$ returns a counterexample which is added to \emph{RED} together with all its prefixes, and all their continuations to  \emph{BLUE} (provided they are not already in \emph{RED}). \\

% Second, for the black-box case we resort to defining a test size based on %PAC\cite{Valiant:1984}. {\color{red} TD: This needs more elaboration.}

%\subsubsection{Implementation considerations}
%In this work we propose a variant of the algorithm in \cite{weiss_WFA_learning} with the following modifications:
%\begin{itemize}
%    \item During the observation table expansion phase, the suffix and prefix thresholds are omitted. That is, no rows are discarded. {\color{red} TD: Could this cause our version to yield worse results (ndcg, etc) than the original with early stopping?}

   % \item  Our PDFA construction algorithm differs from the original implementation in the clustering section (that is built on top of dbscan): we use a greedy clustering technique that performs grouping according to \tol-equality, and then refinement until the WFA is deterministic.
   % The first phase consists in greedily assigning rows to groups, initially we assign the first row in red to a new group, and then for every row in red we find a group where every element is tequal and add it. This is a way of building an initial grouping that holds the t-equality property. Second, 
    
    %\item  The termination criteria was implemented in two ways. First, for the case where the target models are WFAs, we adapt the Hopcroft-Karp algorithm for DFA comparison \cite{hopcroft_karp} to the setting of WFAs, by running a bisimulation on the target and output WFA, and comparing \tol-equivalence of states. Second, for the black-box case we resort to defining a test size based on PAC\cite{Valiant:1984}. {\color{red} TD: This needs more elaboration.}
 %\end{itemize}

%If it terminates, \PLstar\ learns a PDFA $\widehat{\Aut}$ which is \tol-equal to the target PDFA \Aut, that is, $\Aut\tequal_\tol\widehat{\Aut}$. Actually, whenever a counterexample is found, at least one of the prefixes added to \emph{RED} is not \tol-equal to the previous elements of \emph{RED} (otherwise it will not be a counterexample). Thus, at least a new state is discovered, making the number of states to strictly increase at each iteration. {\color{red} FM-SY: Hence, \PLstar\ does terminate.??}

Indeed, following the ideas presented in \cite{maler_pnueli}, it is possible to avoid clustering the set \emph{RED}. Each time a counterexample is found, rather than adding its prefixes to \emph{RED}, its suffixes are added to \Suff. By doing so, there is no need to check for consistency, since the table remains consistent. Therefore, elements from \emph{BLUE} are added to \emph{RED} only to ensure closedness. This happens when for some $p\in BLUE$ there is no $p'\in RED$ s.t. $p \tequal_{\tol}p'$. Thus, for every pair $p_{1},p_{1}'\in RED$, $p_{1}\not\tequal_{\tol}p_{1}'$, which makes clustering unnecessary.
%
With this in mind we developed a column expansion version of \PLstar\ that we called \PLstar\textrm{Col}. %The algorithm was only used to test the effect of clustering on the technique (see \ref{exp:1}).

Fig.~\ref{fig:pdfa_wlstar_vs_quant} (right) shows PDFA $\widehat{\Aut}$ learnt from PDFA \Aut\ (left) with both \PLstar\ and \PLstar\textrm{Col} for $\tol = 0.1$. Notice that $q'_1$ is \tol-equal to $q_1$, $q_2$, and $q_3$, and $q'_2$ is \tol-equal to $q_4$, $q_5$, and $q_6$.\\

\input{assets/pdfa/pdfa_wlstar_vs_quant}

%    \item[Other prop]$\forall p, p' \in RED, \symb \in \Symb$, if $\Clu(p) = \Clu(p')$ then 
%    $\exists p_1, p'_1 \in RED$, $p\symb \tequal_{\Suff,\tol} p_1$, $p'\symb \tequal_{\Suff,\tol} p'_1$, s.t. $\Clu(p_1) = \Clu(p'_1)$.
    


==> assets/algorithms/initialize_observation_tree.tex <==
%\begin{algorithm}[H]
%    \SetKwInOut{Input}{Input}
%    \SetKwInOut{Output}{Output}
%    \SetKwInOut{Parameter}{Parameter}
    
%    \Input{Counterexample $ce$}
%    \Parameter{Quantization Parameter $\kappa$}
%    \Output{N-ary Observation Tree $T$}
    
%    epsilon_child
    
%    \Return T\;
%    \caption{Initialize-Observation-Tree}
%    \label{alg:init-observation-tree}
%\end{algorithm}

==> assets/tables/table_exp_5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}
\caption{----YYY----}
\label{tab:exp_5}
\begin{tabular}{llllccc}
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Target \\ Language\end{tabular}} & \multicolumn{1}{c}{Algorithm} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}WER \\ median\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}NDCG \\ median\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Time (s) \\ median\end{tabular} & \begin{tabular}[c]{@{}c@{}}Exceeded Max \\ Query Length \\ \%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Exceeded Max \\ Number of States \\ \%\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Weighted \\ Tomita 1\end{tabular}}  & QuaNT                         & \textbf{0.0}                                                              & \textbf{1.0}                                                               & 11.63                                                      & 0                                                                          & 0                                                                              \\
                                                                               & WL*                           & \textbf{0.0}                                                              & \textbf{1.0}                                                               & \textbf{5.07}                                              & 0                                                                          & 0                                                                              \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Weighted \\ Tomita 2\end{tabular}}  & QuaNT                         & \textbf{0.29}                                                             & \textbf{0.85}                                                              & 37.20                                                      & 0                                                                          & 100                                                                            \\
                                                                               & WL*                           & 0.69                                                                      & 0.63                                                                       & \textbf{28.11}                                             & 0                                                                          & 0                                                                              \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Weighted \\ Tomita 3\end{tabular}}  & QuaNT                         & \textbf{0.09}                                                             & \textbf{0.96}                                                              & \textbf{24.21}                                             & 100                                                                        & 0                                                                              \\
                                                                               & WL*                           & 0.71                                                                      & 0.59                                                                       & 25.46                                                      & 100                                                                        & 0                                                                              \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Weighted \\ Tomita 4\end{tabular}}  & QuaNT                         & \textbf{0.23}                                                             & \textbf{0.90}                                                              & 53.26                                                      & 0                                                                          & 100                                                                            \\
                                                                               & WL*                           & 0.65                                                                      & 0.67                                                                       & \textbf{21.36}                                             & 100                                                                        & 0                                                                              \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Weighted \\ Tomita 5\end{tabular}}  & QuaNT                         & \textbf{0.23}                                                             & \textbf{0.92}                                                              & 24.32                                                      & 0                                                                          & 100                                                                            \\
                                                                               & WL*                           & 0.37                                                                      & 0.84                                                                       & \textbf{15.61}                                             & 100                                                                        & 0                                                                              \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Weighted \\ Tomita 6\end{tabular}}  & QuaNT                         & \textbf{0.18}                                                             & \textbf{0.94}                                                              & 23.15                                                      & 0                                                                          & 100                                                                            \\
                                                                               & WL*                           & 0.45                                                                      & 0.81                                                                       & \textbf{21.14}                                             & 100                                                                        & 0                                                                              \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Weighted \\ Tomita 7\end{tabular}}  & QuaNT                         & \textbf{0.08}                                                             & \textbf{0.98}                                                              & 29.35                                                      & 0                                                                          & 100                                                                            \\
                                                                               & WL*                           & 0.66                                                                      & 0.68                                                                       & \textbf{24.92}                                             & 100                                                                        & 0                                                                             
\end{tabular}
\end{table}

==> learning.tex <==
%\section{PDFA MAT-learning}\label{pdfa_mat_learning}

%PDFA are MAT-learnable~\cite{beimel_et_al}. However, in constrast to DFA MAT-learning, there are not so many works discussing implementations of algorithms for learning PDFA. One such work is~\cite{weiss_WFA_learning} which proposes \WLstar\ as an adaptation of \Lstar\ to learn \emph{weighted} finite automata (WFA). However, in practice it was tested on PDFA and recurrent neural networks that compute next-symbol distributions over strings. %Other works on learning WFA do not rely on the MAT framework, but rather on spectral learning (e.g.~\cite{ayache_et_al}). 
%In this section, we propose \PLstar, a variant of \WLstar and then introduce \QuaNT.

%\input{WLStar}





==> misc.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[a]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{assets/figures/tomita2.png}
         \caption{}
         \label{fig:tomita2}
     \end{subfigure}%
     \hfill %%
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{assets/figures/tree0_tomita_2.png}
         \caption{}
         \label{fig:tree0_tomita2}
    \end{subfigure}
    \hfill %%
    \caption{(a) Weighted Tomita 2 from \cite{weiss_WFA_learning}. (b) An n-ary tree for this automaton.}
    \label{fig:n_ary_tree_example}
\end{figure}


say
$\widehat{q}_\wor$, associated with access string $\wor\in\AccS$,  $\wor\neq \wor_j = \mathrm{sift}(\ce[j])$, 


% \traW_{\widehat{\Aut}}(\ce[j]) = 
Let $d\in\DisS$ be the least common ancestor in \NTree\ of $\wor$ and $\wor_j$.

By finding such $j$ we know that $\traW_{\widehat{\Aut}}(\ce[j-1]) = \widehat{q}_\wor$, $\wor\in\AccS$,  s.t. $\wor = \wor_{j-1} = \mathrm{sift}(\ce[j])$
but when continued with $\ce_{j}$ they end up in non-equivalent states. This means that $\traW_{\widehat{\Aut}}(\ce[j-1]) \neq \mathrm{sift}(\ce[j-1])$ 


which means that $\policyW_{\Aut}(\ce[j]) \neq_\quantp \policyW_{\widehat{\Aut}}(\ce[j])$, but $\policyW_{\Aut}(\ce[j-1]) =_\quantp \policyW_{\widehat{\Aut}}(\ce[j-1])$.




and $\hat{M}[\ce[j-1]]$ are actually different states but they are in the same equivalence class. To distinguish $\hat{M}[\ce[j-1]]$ from all previously discovered states, we only need to distinguish $M[\ce[j-1]]$ and $\hat{M}[\ce[j-1]]$; in other words, we need to split $\hat{M}[\ce[j-1]]$. Being $d$ the  distinguishing string of the equivalence classes of $M[\ce[j]]$ and $\hat{M}[\ce[j]]$, the distinguishing string for $M[\ce[j-1]]$ and $\hat{M}[\ce[j-1]]$ is  $\ce_{j}d$.



Fig.\ \ref{fig:tomita2} shows a PDFA that will be used as a running example. This automaton, borrowed from \cite{weiss_WFA_learning}, is a PDFA adaptation of automaton Tomita 2 from \cite{tomita}. Fig.\ \ref{fig:n_ary_tree_example} shows an n-ary tree for this PDFA with access strings $\{\emptyW, 0\}$ and distinguishing strings $\{\emptyW\}$. On the edges of the tree, the partition resulting from processing the distinguishing string concatenated with the child node is maintained, and every leaf node maintains the next symbol probabilities of the access string.

\paragraph{Output Model Guarantees}
We will describe some guarantees of the extracted model. Formal definitions and proofs in Appendix??.

\paragraph{Model Determinism} As in WL*\, determinism in the output model is guaranteed by construction, and, if the weights of the target are a probability simplex, then the weights of the output will also be probabilistic.

\paragraph{Equivalence} 
When checking is done by bisimulation, the output and the target are weakly equivalent, that is, both models \emph{quotient} PDFAs are indistinguishable.
On the other hand, if equivalence is reached by a PAC test, the output and the target are probably approximately weakly equivalent with an approximation parameter $\epsilon$ and confidence $1-\delta$.

\paragraph{Progress} 

%\subsubsection{A running example}
%For the running example we will use the PDFA in figure \ref{fig:running_example}. The initialization step will generate the hypothesis present in...

 

-----------------
\\
Secondly, we used some relatively simple LSTM LM-RNNs trained with Weighted Tomitas Grammars from \cite{weiss_WFA_learning} as target systems (Experiment 5).
Finally we evaluate it in a real life case study such as....


==> old_intro.tex <==
Today, deep recurrent neural networks (RNN) are used for language modeling and classification in order to accomplish a variety of safety- and security-critical tasks in a number of application areas, such as autonomous driving~\cite{scheinerADS19, kocic2019end}, intrusion detection~\cite{kim2016long, yin2017deep}, malware detection~\cite{PascanuR15, rhode2017cose, vinayakumar2019robust}, human activity recognition~\cite{singh2017human}, and recently nuclear fusion science~\cite{plasma_control_RL}.
%
Therefore, there is increasing interest in modeling and verifying their behavior with respect to the requirements they must fulfill to correctly perform their task. 
Moreover, taking into consideration the notion of \emph{interpretability} provided in~\cite{miller, biran_and_cotton}, which defines it as the degree to which an observer can understand the cause of a decision, it can be said that  neural networks' nature undermines human capabilities of getting such understanding since their deep and complex architectures, with up to thousands of millions of parameters, makes it impossible for a human to comprehend the rationale of their outputs, even if the underlying mathematical principles are understood and their internal structure and weights are known~\cite{ribeiro}. 

%Moreover, when it comes to interpreting RNN errors, it is useful to do it through an \emph{operational} and \emph{visual} characterization, as a means for gaining insight into the set of incorrect RNN outputs in reasonable time.
\\
For RNN devoted to language modeling (LM-RNNs) one approach to solve these issues is to extract surrogate models or rules from such networks. Recently, works devoting to extract rules from them have been proposed\cite{weiss_WFA_learning, okudono_et_al}. However,  these procedures do not provide quantitative assessments on how precisely the extracted PDFA characterizes the language model of the RNN. 


--------------------------
\\



==> rnn.tex <==
\section{RNN}

Consider the following RNN, for $n\in\Nat, n>0$:
%
\begin{align*}
    h_0 &= 0 \\
    h_n &= 0 \wor_n + h_{n-1} - \varepsilon \text{ for } n>0\\
    o_n &= \mathrm{sigmoid}(h_n)
\end{align*}
%
Suppose the input $\wor \in \Words$, with $\Symb = \{1\}$. Hence, this network is such that $\probP(1|\emptyW) = o_0 = \mathrm{sigmoid}(0) = 0.5$ and $\probP(1|\wor) = o_n = \mathrm{sigmoid}(0.5-n\varepsilon)$. We can naturally extend \probP\ to \SymbT\ with $\probP(\terminal|\emptyW) = 1-o_0 = 0.5$ and $\probP(\terminal|\wor) = 1-o_n = 1-\mathrm{sigmoid}(0.5-n\varepsilon)$. Clearly, this function cannot be computed by a PDFA. That is, there is no equivalent PDFA. Nevertheless, there is a \quantp-equivalent one.

\subsection{Experiment 5}
\label{exp:5}
For this experiment we ran Quant and WL* on LSTM LM-RNNs trained with Weighted Tomitas Grammars from \cite{weiss_WFA_learning} as target systems. The LSTMs have input dimensions 64 and 62 and hidden dimension 30. The LSTMs and their training methods are fully described in \ref{appendix:tomita_lstm}.

The quantization parameter $\kappa$ was fixed in 10, and tolerance $t = 0.1$.
For every instance an algorithm the extraction was ran 10 times.

In this case, both QuaNT and WL* were adapted to use hypothesis complexity bounds as proposed in \cite{MayrYovine}. For this experiment a bound on maximum query length of 20 was set, and a number of states of 10. This is reasonable taking into consideration that the underlying models generating data for the RNN-LM training had at most five states.

It is also important to notice, that having tried a number of configurations, there was to the best of our efforts no way of consistently replicating trainings shown in \cite{weiss_WFA_learning}. This means, extracting PDFAs from the target network that were morphologically similar to the underlying Weighted Tomitas Grammars was a matter of luck. With this in mind, we resorted to use an arbitrary training run and not take into consideration if there was a state explosion phenomenon or if the extracted target had a resemblance to the system generating the traces for the network.

In table \ref{tab:exp_5} WER, NDCG, extraction time median, and percentage of times query length bounds and number of states bounds were exceeded for every instance. As it can be seen QuaNT still manages to avoid exceeding query lenght bounds most of the time while WL* quickly reaches such bounds and terminates. This results in QuaNT extracting PDFAs that yield better error metrics (NDCG and WER) than WL*.\\

\input{assets/tables/table_exp_5}
